Can AI Serve as a Substitute for Human Subjects in Software Engineering Research?

Research within sociotechnical domains, such as Software Engineering, fundamentally requires a thorough consideration of the human perspective. However, traditional qualitative data collection methods suffer from challenges related to scale, labor intensity, and the increasing difficulty of participant recruitment. This vision paper proposes a novel approach to qualitative data collection in software engineering research by harnessing the capabilities of artificial intelligence (AI), especially large language models (LLMs) like ChatGPT. We explore the potential of AI-generated synthetic text as an alternative source of qualitative data, by discussing how LLMs can replicate human responses and behaviors in research settings. We examine the application of AI in automating data collection across various methodologies, including persona-based prompting for interviews, multi-persona dialogue for focus groups, and mega-persona responses for surveys. Additionally, we discuss the prospective development of new foundation models aimed at emulating human behavior in observational studies and user evaluations. By simulating human interaction and feedback, these AI models could offer scalable and efficient means of data generation, while providing insights into human attitudes, experiences, and performance. We discuss several open problems and research opportunities to implement this vision and conclude that while AI could augment aspects of data gathering in software engineering research, it cannot replace the nuanced, empathetic understanding inherent in human subjects in some cases, and an integrated approach where both AI and human-generated data coexist will likely yield the most effective outcomes.

==> cover_letter.tex <==
Dear Editors,

I am writing to submit the manuscript "Can AI Serve as a Substitute for Human Subjects in Software Engineering Research?" on behalf of my co-authors for consideration in the vision track on the future of qualitative research in Automated Software Engineering.

This vision paper explores whether AI models like ChatGPT could potentially replace human participants in qualitative SE research. The authors propose leveraging techniques like persona-based prompting to allow large language models to simulate diverse human responses and behaviors, generating text and data that provide insights into user attitudes and experiences.

While noting ethical concerns, the authors thoughtfully discuss the prospect of an integrated methodology combining AI-generated and human data to optimize outcomes. This forward-looking work makes a valuable contribution by conceptualizing new frontiers for AI in qualitative SE research that can have a profound influence. I believe this article would strongly resonate with ASE readers.

Thank you for considering this timely and intriguing manuscript. I'm happy to provide any additional information needed during review. I look forward to your decision.




Sincerely,
